State-of-Charge Targets for Storage Participation in Two-Settlement Markets: Reliability, Price, and Compensation Impacts

As energy storage assumes a larger role in electricity systems, market operation must coordinate its use across time to support reliability during periods of system stress. Minimum state-of-charge (SOC) targets provide a means of preserving energy for these periods, but their design shapes reliability, operating efficiency, and storage compensation. This paper evaluates alternative SOC target designs in a California-based day-ahead and real-time electricity market model. The comparison examines targets based on day-ahead schedules or rolling centralized dispatch, enforced at the individual-resource or system level, across seasons, stress conditions, and participant information settings. The results show that retaining more energy does not necessarily reduce load shedding: targets that restrict discharge can limit storage support during shortages. Under critical summer conditions, individual targets derived from rolling centralized dispatch reduce weekly load shedding by approximately 83--84\% relative to operation without targets. Lower RT clearing costs and average prices can coexist with higher storage compensation, reflecting the role of day-ahead positions and real-time deviations in determining settlement outcomes. These findings highlight the importance of coordinating energy retention with timely discharge and network deliverability when designing SOC requirements for storage participation in electricity markets.

==> sections/stress_sensitivity_framework.tex <==
\subsection{Sensitivity to Net-Load Stress}\label{sec:stress-sensitivity}

The representative-day analysis shows how an every-period SOC floor can
restrict energy release during a shortage. The sensitivity experiments
extend this analysis to increasing system stress, examining both the
benefits and the operating limits of the target designs. Two summer
sweeps are considered: a demand perturbation and a joint perturbation of
demand and renewable availability. Generation, storage, and transmission
capacities remain fixed. Outcomes are evaluated over the same seven-day
window, with Aligned and Limited settings reported separately. The focus
here is the response to stress within each setting.

\textit{[Draft framework: numerical results, plotted trajectories, and
comparative conclusions will be inserted after the final run audit. All
TBD entries below denote pending results, not zero outcomes or infeasibility.]}

\subsubsection{Reliability and Cost under Increasing Demand}
The demand sweep increases the configured peak-demand perturbation from
the baseline through successive stress levels. Its within-day profile
and associated spatial transfer vary with the level, so the horizontal
axis represents the configured perturbation rather than a uniform
increase in demand at every bus and interval. Weekly load shedding and RT clearing
cost are compared at each level using complete weeks for the relevant
strategies. Figure~\ref{fig:stress-framework} reserves separate views for
the two sweeps; Table~\ref{tab:stress-framework} provides the format for
selected high-stress comparisons.

The reliability comparison examines how load shedding grows with stress and whether
the target designs reduce shortages relative to No target. Absolute load shedding
is reported alongside changes from the baseline strategy so that small
low-stress events remain visible. Percentage reductions are used only
when the corresponding No-target load shedding is positive. The cost comparison
uses the same cases and weekly horizon; RT clearing cost includes the
load shedding penalty and is not interpreted as a separate measure of
physical production cost or social welfare.

\textit{[Results to insert: low-stress behavior and exceptions; load shedding and
cost changes at intermediate and high stress; residual load shedding at the highest
completed level. State the supported trend and its exceptions without
assuming a common strategy ranking across levels.]}

\begin{figure*}[!t]
\centering
\fbox{\begin{minipage}[c][1.05in][c]{0.46\textwidth}
\centering\small
\textbf{Demand sensitivity}\\[5pt]
Weekly load shedding and RT clearing cost\\
versus configured peak-demand uplift\\[5pt]
Aligned and Limited panels\\
\textit{Curves pending final results}
\end{minipage}}\hfill
\fbox{\begin{minipage}[c][1.05in][c]{0.46\textwidth}
\centering\small
\textbf{Joint net-load sensitivity}\\[5pt]
Weekly load shedding and RT clearing cost\\
versus calibrated net-load stress\\[5pt]
Aligned and Limited panels\\
\textit{Curves pending final results}
\end{minipage}}
\caption{Reserved sensitivity-figure layout. Each experiment will show
weekly load shedding and RT clearing cost separately by information setting.
The two stress axes have different calibration definitions and are not
numerically interchangeable. Only validated complete-week outcomes will
be plotted; unavailable results will be identified separately.}
\label{fig:stress-framework}
\end{figure*}

\subsubsection{Joint Demand and Renewable Stress}
The joint sweep changes nodal demand and solar/wind availability together
along the deviation from native RT conditions to a critical reference.
Its levels are calibrated using the difference between the independent
RT and DA net-load peaks on the reference day. The calibration coefficient
then applies across the week; other days need not attain the reference-day
percentage. Consequently, equal numerical levels in the demand and joint
sweeps do not represent equivalent operating conditions.

This comparison examines whether the patterns observed in the demand
sweep also occur when increased demand is accompanied by changes in
renewable availability. Particular attention is given to any reversal
in the relative performance of DA and CD targets, and to shortages that
persist despite retained storage energy. Interpretation follows the
release mechanism in Section~\ref{sec:daily-mechanism}, with additional
trajectory analysis where needed to support an explanation.

\textit{[Results to insert: complete-week load shedding and cost comparisons at the
selected joint-stress levels; whether the demand-sweep findings persist;
any DA-target deterioration or low-stress exceptions supported by the
final data.]}

\begin{table*}[!t]
\centering
\caption{Template for a selected high-stress comparison. Experiment,
information setting, and stress level: TBD. Repeat this block for the
selected conditions after validation. Changes are measured relative to
No target within the same condition; TBD denotes a pending value.}
\label{tab:stress-framework}
\small
\setlength{\tabcolsep}{10pt}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Strategy & load shedding (MWh) & load shedding change (MWh) & RT cost (USD million) & Cost change (\%) \\
\midrule
No target & TBD & --- & TBD & --- \\
DA individual & TBD & TBD & TBD & TBD \\
DA system & TBD & TBD & TBD & TBD \\
CD individual & TBD & TBD & TBD & TBD \\
CD system & TBD & TBD & TBD & TBD \\
\bottomrule
\end{tabular}
\end{table*}

\subsubsection{Target Granularity and Operating Limits}
Comparing CD individual with CD system assesses how resource-specific
energy floors and an aggregate requirement perform as stress increases.
The comparison includes both reliability and cost, allowing the two
metrics to favor different designs. Because the CD formulations also
differ in their scenario envelopes and interpolation anchors, observed
differences are interpreted as outcomes of the implemented designs rather
than enforcement granularity alone.

At the upper end of each sweep, residual load shedding is used to assess the limits
of energy management with fixed physical capacities. Residual shortages
alone do not identify their cause: binding energy floors, available
discharge power, conventional supply, and network constraints must be
distinguished using the operating results. Complete-week comparisons
exclude partial runs. A verified infeasible solve is reported separately
from an unfinished or unavailable run. The effective-input and bid-update
differences described above remain relevant to comparisons across
strategies.

\textit{[Conclusions to insert: the conditions under which each CD design
performs better; any reliability--cost tradeoff; the remaining shortages
at high stress; and the target-design implication supported jointly by
the sensitivity results and the representative-day mechanism.]}


==> tables/demand-sensitivity.tex <==
% Generated by tools/build_results_tables.py.
\begin{table}[!htb]
\centering
\caption{Weekly demand-stress sensitivity. Load shedding is in MWh; RT cost is in USD million. N: No target; D: DA individual; C: CD individual.}\label{tab:demand-sensitivity}
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
 & & \multicolumn{3}{c}{Load shedding} & \multicolumn{3}{c}{RT cost} \\ \cmidrule(lr){3-5}\cmidrule(lr){6-8}Info. & Level (\%) & N & D & C & N & D & C \\
\midrule
Aligned & 0 & 1.55 & 0.00 & 14.47 & 90.87 & 90.95 & 90.31 \\
 & 2 & 0.00 & 0.00 & 1.72 & 93.26 & 93.22 & 92.45 \\
 & 4 & 2.34 & 0.00 & 0.00 & 95.61 & 95.62 & 94.75 \\
 & 6 & 37.96 & 2.62 & 8.31 & 98.03 & 97.99 & 97.01 \\
 & 8 & 7,082.75 & 2,319.08 & 58.53 & 114.16 & 104.93 & 99.63 \\
 & 10 & 19,574.26 & 9,545.77 & 415.70 & 140.70 & 121.33 & 102.66 \\
 & 12 & 37,493.05 & 22,912.02 & 6,507.21 & 177.60 & 149.63 & 134.18 \\
\midrule
Limited & 0 & 0.00 & 0.00 & 1.64 & 90.88 & 90.95 & 90.35 \\
 & 2 & 0.00 & 0.00 & 0.00 & 93.27 & 93.27 & 92.75 \\
 & 4 & 3.48 & 0.00 & 0.00 & 95.58 & 95.60 & 94.98 \\
 & 6 & 1,125.83 & 2.49 & 0.00 & 100.24 & 98.01 & 97.20 \\
 & 8 & 7,237.72 & 2,228.46 & 31.21 & 114.38 & 104.82 & 99.60 \\
 & 10 & 19,463.58 & 10,244.36 & 343.00 & 140.38 & 122.73 & 105.99 \\
 & 12 & 38,296.89 & 23,301.25 & 7,408.78 & 179.15 & 150.44 & 132.62 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/joint-sensitivity.tex <==
% Generated by tools/build_results_tables.py.
\begin{table}[!htb]
\centering
\caption{Weekly joint demand/renewable sensitivity. Load shedding is in MWh; RT cost is in USD million. N: No target; D: DA individual; C: CD individual.}\label{tab:joint-sensitivity}
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
 & & \multicolumn{3}{c}{Load shedding} & \multicolumn{3}{c}{RT cost} \\ \cmidrule(lr){3-5}\cmidrule(lr){6-8}Info. & Level (\%) & N & D & C & N & D & C \\
\midrule
Aligned & 0 & 0.00 & 0.00 & 0.00 & 88.99 & 89.26 & 88.99 \\
 & 2 & 0.00 & 0.00 & 0.00 & 89.60 & 89.83 & 89.27 \\
 & 4 & 0.00 & 0.00 & 0.00 & 91.15 & 91.18 & 90.62 \\
 & 6 & 0.00 & 0.00 & 1.28 & 92.49 & 92.65 & 91.81 \\
 & 8 & 0.00 & 0.00 & 0.00 & 93.98 & 94.15 & 93.27 \\
 & 10 & 309.59 & 726.55 & 0.00 & 96.04 & 97.13 & 94.65 \\
 & 12 & 4,476.13 & 4,776.76 & 226.68 & 105.57 & 106.46 & 96.77 \\
\midrule
Limited & 0 & 0.00 & 0.00 & 1.92 & 88.99 & 89.25 & 88.80 \\
 & 2 & 0.00 & 0.00 & 1.59 & 89.63 & 89.81 & 89.35 \\
 & 4 & 0.00 & 0.00 & 0.00 & 91.04 & 91.20 & 90.66 \\
 & 6 & 0.00 & 0.00 & 0.00 & 92.55 & 92.69 & 92.03 \\
 & 8 & 0.00 & 0.00 & 0.00 & 93.95 & 94.16 & 93.44 \\
 & 10 & 596.96 & 560.72 & 0.00 & 96.59 & 96.86 & 94.95 \\
 & 12 & 2,477.78 & 4,505.49 & 144.57 & 101.67 & 105.99 & 96.53 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/seasonal_overview.tex <==
% Generated by tools/build_seasonal_overview.py from complete weekly records.
\begin{table*}[!t]
\centering
\caption{Four-season completion and paired comparisons with No target.
Cost and load shedding comparisons use only groups with a complete seven-day result
for both strategies. Median cost change is the median of
$100(C_s-C_0)/C_0$ across those groups, where $C_0$ is No-target RT
clearing cost. Load shedding columns count groups; their sum equals the number of
complete groups. Different strategies have different comparison subsets.}
\label{tab:seasonal-summary}
\small
\setlength{\tabcolsep}{8pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
 & Complete & Lower RT & Median cost & \multicolumn{3}{c}{load shedding versus No target} \\
\cmidrule(l){5-7}
Strategy & groups & cost & change & Lower & Unchanged & Higher \\
\midrule
No target & 16/16 & --- & --- & --- & --- & --- \\
DA individual & 15/16 & 11/15 & $-0.70\%$ & 2 & 10 & 3 \\
DA system & 2/16 & 2/2 & $-8.99\%$ & 1 & 1 & 0 \\
CD individual & 16/16 & 15/16 & $-2.02\%$ & 4 & 11 & 1 \\
CD system & 14/16 & 12/14 & $-1.29\%$ & 2 & 11 & 1 \\
\bottomrule
\end{tabular}
\end{table*}

